Adaptive Local Bayesian Optimization Over Multiple Discrete Variables

In the machine learning algorithms, the choice of the hyperparameter is often an art more than a science, requiring labor-intensive search with expert experience. Therefore, automation on hyperparameter optimization to exclude human intervention is a great appeal, especially for the black-box functions. Recently, there have been increasing demands of solving such concealed tasks for better generalization, though the task-dependent issue is not easy to solve. The Black-Box Optimization challenge (NeurIPS 2020) required competitors to build a robust black-box optimizer across different domains of standard machine learning problems. This paper describes the approach of team KAIST OSI in a step-wise manner, which outperforms the baseline algorithms by up to +20.39%. We first strengthen the local Bayesian search under the concept of region reliability. Then, we design a combinatorial kernel for a Gaussian process kernel. In a similar vein, we combine the methodology of Bayesian and multi-armed bandit,(MAB) approach to select the values with the consideration of the variable types; the real and integer variables are with Bayesian, while the boolean and categorical variables are with MAB. Empirical evaluations demonstrate that our method outperforms the existing methods across different tasks.

==> tex/4_conclusion.tex <==
\section{Conclusion and Future Works}

%Although the TuRBO has shown its competence on hyperparameter optimization by local searching, the consideration on realistic, general setting of configurations is left behind, consequently dropping its potential.

In this paper, we introduced our methods to challenge the NeurIPS 2020 BBO competition by enhancing TuRBO. We managed to \textit{(1)} impose adaptive partitioning for the local modeling to guide the sampling toward the promising region; \textit{(2)} treat discrete variables with sophisticatedly designed kernels; \textit{(3)} combining multi-armed bandit approach to replace values for categorical and boolean variables.
%which distinctively possess different characteristics comparing to continuous variable. 
%Through adaptively partitioning we filtered out unnecessary samples to make the most of our evaluation budget. By introducing a new, sophisticatedly designed kernel, we let the surrogate model effectively learn not only the intrinsic behavior of different variable types, but also an accurate interaction between them. Lastly, by combining multi-armed bandit approach to generate values of categorical and boolean variables, it made an effect of exposing a bit of scattering from the bounded region so that the search can also take an explorative choice.


%We have mainly focused on treating the discrete variables which distinctively possess different characteristics comparing to continuous variables. By introducing a new, sophisticatedly designed kernel, we let the surrogate model effectively learn not only the intrinsic behavior of different variable types, but also an accurate interaction between them. Furthermore, by combining multi-armed bandit approach to generate values of categorical and boolean variables, it made an effect of exposing a bit of scattering from the bounded region so that the search can also take an explorative choice.

Our approach numerically proved its improvement comparing to the baseline. As a future work, a theoretical analysis on the remarkable performance of local search can be expected. 

%Moreover, extending the learning space partition to multiple trust regions can also be another direction of study. 

